How Much is 131 Million Dollars? Putting Numbers in Perspective with Compositional Descriptions

How much is 131 million US dollars? To help readers put such numbers in context, we propose a new task of automatically generating short descriptions known as perspectives, e.g. "$131 million is about the cost to employ everyone in Texas over a lunch period". First, we collect a dataset of numeric mentions in news articles, where each mention is labeled with a set of rated perspectives. We then propose a system to generate these descriptions consisting of two steps: formula construction and description generation. In construction, we compose formulae from numeric facts in a knowledge base and rank the resulting formulas based on familiarity, numeric proximity and semantic compatibility. In generation, we convert a formula into natural language using a sequence-to-sequence recurrent neural network. Our system obtains a 15.2% F1 improvement over a non-compositional baseline at formula construction and a 12.5 BLEU point improvement over a baseline description generation.

==> experiments.tex <==
\section{End-to-End Evaluation}
\label{sec:experiments}

In \refsecs{selection}{generation},
we evaluated the individual components of our perspective generation system.
We now present results from an end-to-end evaluation.

% dataset 
\paragraph{Setup.}
We use a separate collection of 225 sentences (25 sentences for each of 9 units) containing a numeric mention with a value that is greater than 20 or less than 0.1.
\pl{We should have better names - how about SingleFact, Comp-Rule, Comp-Learn?}
We compared three systems: 
\begin{itemize}
  \item \textsc{baseline}: a non-compositional baseline that constructs formulae using a single tuple from the knowledge base that is numerically closest to the mentioned value.
  \item \textsc{generation-baseline}: a system that constructs compositional formula from the knowledge base using familiarity and proximity features, but generates perspectives using the simple rule-based method from \refsec{generation}). 
  \item \textsc{system}: our full system that constructs compositional formula as described in \refsec{selection} and generates perspectives using the sequence-to-sequence model described in \refsec{generation}. 
\end{itemize}
For each mention, we chose the top three perspectives generated by each system. 

\pl{say that we're interested in evaluating selection and generation quality,
but also in framing (a bonus)}
To evaluate the generated perspectives, we showed each mention and perspective to five crowdworkers,
following which they were asked to rate the perspective on a 5-point Likert scale (\reffig{eval-task}):
\begin{enumerate}
  \setlength\itemsep{0pt}
  \item After reading the description, did the quantity described seem smaller or larger than you first thought?
  \item Was the description helpful in understanding the scale of the quantity mentioned?
  \item Was the description appropriate or on topic for the sentence?
\end{enumerate}

%The first question was included to get information to understand how perspectives frame the mentioned quantities.
%The second question is the root of 
%The choice of an appropriate perspective is quite subjective and is an interesting to study framing.
%This is a subjective task

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=\columnwidth]{figures/eval-zoomed}
  \end{center}
  \caption{\label{fig:eval-task} 
  A screenshot of the crowdsourced task to evaluate the quality of the generated perspectives.}
\end{figure}

\paragraph{Results.}
\reftab{results-end2end} summarize the overall usefulness ratings of our system
and \reffig{examples-end2end} provide some examples of our output.

\begin{table*}
  \begin{center}
    \input end2end.table
  \end{center}
  \caption{\label{tab:results-end2end} }
\end{table*}

\begin{table*}
  \begin{center}
    \input end2end.examples
  \end{center}
  \caption{\label{tab:examples-end2end} Some examples of useful output generated by our system.}
\end{table*}

\ac{Discuss breakdown of results.}
\ac{When does compositionality help?}
\ac{When does relevance matter?}
\ac{What happens with framing?}

\pl{realistically due to time and space, this is probably going to be just one paragraph}

